A Strontium-rich Ultra Metal-poor Star in the Atari Disk Component

We report on the discovery of the first ultra metal-poor (UMP) star 2MASS~J20500194$-$6613298 (J2050$-$6613; \mbox{[Fe/H] = $-4.05$}) selected from the Gaia BP/RP spectral catalog that belongs to the ancient Atari disk component. We obtained a high-resolution spectrum for the star with the MIKE spectrograph on the Magellan-Clay telescope. J2050$-$6613 displays a typical chemical abundance pattern for UMP stars, including carbon and zinc enhancements. In contrast, J2050$-$6613 shows extremely high [Sr/Fe] and [Sr/Ba] ratios compared to other stars in the [Fe/H] $<-4.0$ regime. J2050$-$6613 is most likely an early Population\,II star that formed from a gas cloud that was chemically enriched by a massive Population\,III hypernova (E $> 10^{52}$\,erg). Such a Population\,III core-collapse hypernova could simultaneously explain the origin of the abundance pattern of light and heavy elements of 2MASS~J2050$-$6613 if a large amount of Sr of $\sim10^{-5}$\,M$_{\odot}$ was produced, possibly by neutrino-driven \textbf{(wind)} ejecta. Therefore, the abundance pattern of 2MASS~J2050$-$6613 places important constraints on Sr-producing nucleosynthesis sources operating in the Atari progenitor at the earliest times.

==> tables/tab1.tex <==
\begin{table*}
\caption{Basic Observational Data for J2050$-$6613}
\label{tab:candlist}
\begin{tabular}{lcccl}
\hline
\hline
Quantity & Symbol & Value & Units & Reference \\
Right ascension           & $\alpha$ (J2000)    & 20:50:01.95         & hh:mm:ss.ss   & Simbad                                               \\
Declination               & $\delta$ (J2000)    & $-$66:13:29.75      & dd:mm:ss.s    & Simbad                                               \\
Galactic longitude        & $\ell$              & 328.77              & degrees       & Simbad                                               \\
Galactic latitude         & $b$                 & $-$36.49            & degrees       & Simbad                                               \\
Gaia DR3 Name             &                     & 6425379106130933376 &               & \citet{Gaia_DR3}                                     \\
$B$ magnitude             & $B$                 & 13.781 $\pm$ 0.010  & mag           & \citet{UCAC}                                         \\
$V$ magnitude             & $V$                 & 13.119 $\pm$ 0.010  & mag           & \citet{UCAC}                                         \\
$J$ magnitude             & $J$                 & 11.601 $\pm$ 0.021  & mag           & \citet{UCAC}                                         \\
$H$ magnitude             & $H$                 & 11.159 $\pm$ 0.025  & mag           & \citet{UCAC}                                         \\
$K$ magnitude             & $K$                 & 11.083 $\pm$ 0.021  & mag           & \citet{UCAC}                                         \\ 
Color excess              & $E(B-V)$            & 0.0396 $\pm$ 0.001  & mag           & \citet{schlafly2011}                                 \\
Bolometric correction     & BC$_V$              & $-$0.54 $\pm$ 0.08  & mag           & \citet{casagrande2014}                               \\
Radial velocities         & RV                  & 197.32 $\pm  2.04$  & \kmsec        & Gaia DR3 \citep{Gaia_EDR3}                           \\
                          &                     & 196.50 $\pm  4.18$  & \kmsec        & RAVE \citep{RAVE_5th}                                \\
                          &                     & 196.10 $\pm  4.28$  & \kmsec        & RAVE \citep{RAVE_6th}                                \\
                          &                     & 195.59 $\pm  0.50$   & \kmsec       & Magellan (MJD: 60056.41)                             \\
Effective Temperature     & \teff               & 5000 $\pm$ 100      & K             & \citet{Gaia_DR3}                                     \\
Log of surface gravity    & \logg               & 1.80 $\pm$ 0.30     & (cgs)         & This study (Magellan)                                \\
Microturbulent velocity   & v$_{\text{micro}}$  & 1.39 $\pm$ 0.30     & \kmsec        & This study (Magellan)                                \\
Metallicity               & \metal              & $-$4.05 $\pm$ 0.20  & dex           & This study (Magellan)                                \\
\hline
\end{tabular}
\end{table*}

